A Bayesian Model of Dose-Response for Cancer Drug Studies

Exploratory cancer drug studies test multiple tumor cell lines against multiple candidate drugs. The goal in each paired (cell line, drug) experiment is to map out the dose-response curve of the cell line as the dose level of the drug increases. We propose Bayesian Tensor Filtering (BTF), a hierarchical Bayesian model for dose-response modeling in multi-sample, multi-treatment cancer drug studies. BTF uses low-dimensional embeddings to share statistical strength between similar drugs and similar cell lines. Structured shrinkage priors in BTF encourage smoothness in the dose-response curves while remaining adaptive to sharp jumps when the data call for it. We focus on a pair of cancer drug studies exhibiting a particular pathology in their experimental design, leading us to a non-conjugate monotone mixture-of-Gammas likelihood. To perform posterior inference, we develop a variant of the elliptical slice sampling algorithm for sampling from linearly-constrained multivariate normal priors with non-conjugate likelihoods. In benchmarks, BTF outperforms state-of-the-art methods for covariance regression and dynamic Poisson matrix factorization. On the two cancer drug studies, BTF outperforms the current standard approach in biology and reveals potential new biomarkers of drug sensitivity in cancer. Code is available at https://github.com/tansey/functionalmf.

==> doseresponse.tex <==
% !TEX root = aoas.tex
\section{Bayesian dose-response model for cancer drug studies}
\label{sec:dose-response}
The BTF model is a general framework for functional matrix factorization. To apply this framework to dose-response data requires an extra set of modeling steps on top of BTF. Here we describe the cancer drug experiments in detail and an empirical Bayes procedure to estimate the observation likelihood in the face of technical error.

We describe the dose-response model in the context of the specific protocol used for the internal pilot study at Columbia University Medical Center. The second study we analyze uses a different protocol with a different number of plates, wells per plate, concentrations, replications, and other experimental designs. These distinctions are changes to the dimensions of the resulting tensor, but the fundamental statistical inference technique remains the same. We use the same method to analyze and compare both datasets in \cref{sec:results}.

\begin{figure}[t]
\centering
\begin{subfigure}{0.47\linewidth}\includegraphics[width=\linewidth]{figures/experiment-design.pdf}\caption{\label{fig:plate} Experimental design}\end{subfigure}
\begin{subfigure}{0.47\linewidth}\includegraphics[width=\linewidth]{figures/empirical-bayes-means.pdf}\caption{\label{fig:empirical-bayes} Empirical Bayes estimate}\end{subfigure}
\caption{\label{fig:dose-setup} Left: The layout of each microwell plate experiment used to generate a single functional matrix entry. Cells are pipetted one column at a time, leading to correlated errors. Right: Estimate of the prior distribution of mean cell counts in each column, relative to the control column mean. The prior is estimated empirically assuming the lowest concentration had no effect if it had a higher mean.}
\end{figure} 

\subsection{Experimental design and technical error}
\label{subsec:dose-response:experiment}
Each functional matrix entry is derived from a microwell plate experiment where a drug is tested against a biological sample. Each experiment measures cell counts after applying the drug at $9$ different concentrations. The cell counts are measured relative to a baseline control population where no drug was applied. For the control and each concentration level, $6$ replicates are tested. \Cref{fig:plate} shows the design of each $60$-well plate experiment. All experiments are normalized by dividing the population size estimates at each concentration by the control mean for the plate.

% \subsection{Technical bias and correlated errors due to pipetting}
% \label{subsec:dose-response:pipetting}
The first step in each experiment is to pipette an initial population of cells into each of the $60$ microwells on the plate. This is a time consuming process for the biologist, often taking hours to pipette a single plate. To speed up the plating process, biologists use a multi-headed pipette that enables them to simultaneously fill an entire column of each plate. This reduces the burden on the biologist, but comes at a cost: correlated errors.

When a biologist fills a microwell, they first draw a pool of cells into the pipette. Given the small volumes involved in laboratory experiments, the actual number of cells drawn can vary substantially on a relative basis. Using a multi-headed pipette transforms this variation into a hierarchical model: first a pool of cells is drawn into the pipette, then it is split among all the heads. The majority of the variation comes in the initial sampling, with small noise added in the splitting process. This has the unintended side effect of creating correlated errors between all microwells in a single column.

\subsection{Empirical Bayes likelihood estimation}
\label{subsec:dose-response:likelihood}
The correlated errors in the columns render the exact effects unidentifiable. Each column has two latent variables affecting the final population size of cells: a dose-level effect from the drug and an initial population size from the pipetting. Since both of these variables affect all replicates in a column, disentangling them precisely is impossible. Nevertheless, an estimate of dose-response must be provided.

We take an empirical Bayes approach to disentangling the variation in drug effects from the technical error in pipetting. In most experiments, the lowest concentration tested is too small to have any effect on cell survival. We therefore make the assumption that any experiment where the mean of the control replicates is lower than the mean of the replicates treated at the lowest concentration has effectively two sets of control columns. This enables estimation of the variation between means and form an empirical Bayes prior for the pipetting error.

Specifically, we form a histogram of all lowest-concentration means greater than the control mean on the same plate. We then fit a Poisson GLM with $3$ degrees of freedom to the histogram to estimate the prior probability that the mean of the initial population of cells was higher than the control mean. We then assume the true distribution is symmetric and obtain an empirical Bayes prior on the means. \Cref{fig:empirical-bayes} shows an example histogram and empirical Bayes prior estimate. The within-column variance is identifiable and estimated using the controls. The empirical Bayes likelihood is then a gamma mixture model that integrates out the uncertainty in the initial population mean,
\begin{equation}
\label{eqn:empirical_bayes_likelihood}
P(y_{ijt} \mid w_i^\top v_{jt}) = \prod_{r=1}^{R} \left( \sum_{k=1}^{K} \hat{m}_k Ga(y_{ijtr}; \hat{a}_k, \hat{b}_k w_i^\top v_{jt}) \right) \mathds{1}[0 \leq w_i^\top v_{jt} \leq 1] \, ,
\end{equation}
where $(\hat{m}, \hat{a}, \hat{b})_k$ are the weights derived from the empirical Bayes procedure. The scale regression form of the inner product is due to the property that the gamma random variable is being multiplied by the effect of the drug. That is, the population of cells is being killed at some latent rate. The inner product is constrained to be a proportion, as the drugs are known not to help any cells grow (i.e., the proportion must be at most $1$) and a drug cannot kill more than all of the cells. The likelihood in \cref{eqn:empirical_bayes_likelihood} is non-conjugate to the BTF hierarchical model and thus we use the generalized elliptical slice sampling routine from \Cref{sec:gass} for inference.




